Pseudo-Label Enhanced Prototypical Contrastive Learning for Uniformed Intent Discovery

New intent discovery is a crucial capability for task-oriented dialogue systems. Existing methods focus on transferring in-domain (IND) prior knowledge to out-of-domain (OOD) data through pre-training and clustering stages. They either handle the two processes in a pipeline manner, which exhibits a gap between intent representation and clustering process or use typical contrastive clustering that overlooks the potential supervised signals from the whole data. Besides, they often individually deal with open intent discovery or OOD settings. To this end, we propose a Pseudo-Label enhanced Prototypical Contrastive Learning (PLPCL) model for uniformed intent discovery. We iteratively utilize pseudo-labels to explore potential positive/negative samples for contrastive learning and bridge the gap between representation and clustering. To enable better knowledge transfer, we design a prototype learning method integrating the supervised and pseudo signals from IND and OOD samples. In addition, our method has been proven effective in two different settings of discovering new intents. Experiments on three benchmark datasets and two task settings demonstrate the effectiveness of our approach.

==> intro_old.tex <==
\section{Introduction}
%\IEEEPARstart {U}{nderstanding} intent is essential as it determines how the system responds accurately to the user's requests. By accurately identifying the user's intent, the dialogue system can better comprehend the user's needs and provide appropriate responses or execute the corresponding tasks. Intent discovery has received a surge of attention due to its crucial role in dialogue systems\cite{vedula2019towards},\cite{min2020dialogue}. This task requires the model to learn new concepts automatically without manual annotation or supervision.

%Task-oriented dialogue systems play a pivotal role in diverse applications, guiding users to achieve specific goals through natural language interactions, such as booking a restaurant, managing bank transactions \textit{etc} \cite{louvan2020recent,wu2022state}. The task of user intent understanding has garnered substantial attention due to its pivotal role in enabling the system to comprehend user needs \cite{vedula2019towards, min2020dialogue}. While traditional supervised methods have exhibited remarkable performance in this task, their limitations include the recognition of only pre-defined in-domain (IND) intent categories and the requirement of a significant amount of labeled training data, which is both laborious and expensive to obtain. In real-world scenarios, new unseen intents , which are also called out-of-domain (OOD) intents, will emerge after the deployment of dialogue systems, posing challenges for supervised intent classification methods. Therefore, the intent discovery task becomes increasingly critical, focusing on uncovering and categorizing new intents not present in the training data.
Intent discovery has received increasing attention due to its crucial role in dialogue systems\cite{vedula2019towards,min2020dialogue}. %Understanding the user's intent is paramount as it determines how the system responds accurately to the user's requests. 
By accurately identifying the user's intent, the system can better comprehend the user's needs and provide appropriate responses or execute the corresponding tasks. 

For intent discovery, researchers have delved into unsupervised methods, which are characterized by clustering on out-of-domain (OOD) data without incorporating prior knowledge of in-domain (IND) data \cite{hakkani2015clustering,shi2018auto,liu2021open}. However, in real-world scenarios, it is more common to have access to a limited amount of labeled data, rather than dealing with entirely unlabeled datasets. Consequently, recent research endeavors have shifted towards the semi-supervised setting which can be broadly categorized into OOD intent discovery and open intent discovery \cite{mou2022disentangled,mou2022watch,lin2020discovering,zhang2021discovering,shen2021semi,zhang2022new}. As shown in Figure \ref{setting}, OOD intent discovery aims to cluster solely unlabeled OOD intents by leveraging sufficient labeled IND prior knowledge. In contrast, open intent discovery aims to recognize both known and new categories from unlabeled data.

%In this paradigm, the approach involves initial pre-training of an in-domain intent classifier. Subsequently, clustering algorithms are applied to the extracted OOD intent representations obtained from the pre-trained in-domain intent classifier. This innovative methodology demonstrates a more nuanced and effective approach to handling out-of-distribution instances, considering the contextual understanding gained from in-domain data.


%Existing works in intent discovery can be broadly categorized into open intent discovery and out-of-domain (OOD) intent discovery. Open intent discovery focuses on clustering both IND and OOD intents using limited IND information. On the other hand, OOD intent discovery aims to cluster OOD intents by leveraging sufficient IND prior knowledge. Both of these settings significantly contribute to improving the performance and portability of task-oriented dialogue systems.%, while previous work only cater to one and often have limited generalization.
\iffalse
\begin{figure}[t]
    \centering
    \centering
    \subfigure[Open-setting]{
        \includegraphics[scale=0.06]{settings1.5.png}
    }
    % \subfigure[CE+CC]{
    %     \includegraphics[scale=0.5]{fig/CE+CC_end.pdf}
    % }
    \subfigure[OOD-setting]{
        \includegraphics[scale=0.06]{settings2.5.png}
    }
   
    %\vspace{-0.45cm}
    \caption{Two basic task setting for intent discovery. %For open-setting, only a portion of IND data in training set is labeled, and the test set includes all categories (IND and OOD). In the OOD setting, all IND data is labeled, and the test set only includes OOD categories. 
    In open-setting: Partially labeled IND data for training, all categories in test (IND and OOD). In OOD setting: Fully labeled IND data for training, only OOD categories in test.
    }
    \label{Effect of KCC}
    %\vspace{-0.5cm}
\end{figure}
\fi


\begin{figure}[t]
    \centering
    \centering
   \includegraphics[height=0.22\textwidth]{img/our_settings.png}
    %\vspace{-0.45cm}
    \caption{Two basic task setting for intent discovery. %For open-setting, only a portion of IND data in training set is labeled, and the test set includes all categories (IND and OOD). In the OOD setting, all IND data is labeled, and the test set only includes OOD categories. 
    In open-setting: Partially labeled IND data for training, all categories in test (IND and OOD). In OOD setting: Fully labeled IND data for training, only OOD categories in test.
    }
    \label{setting}
    %\vspace{-0.5cm}
\end{figure}


%\yx{briefly introduce Fig.1}
%Figure 1 illustrates the key distinctions between the two basic settings. Open Intent discovery is focused on an open scenario where emerging samples may belong to both IND (In-Domain) and OOD (Out-of-Domain) categories, while OOD intent discovery is based on sufficient IND prior knowledge and aims to address the challenge of migrating the system to a completely new scenario, involving unsupervised clustering objectives specifically designed for clustering only OOD intents.

%\yx{2nd paragraph: introduce related work with high-level, such as: the existing works can be divided into xx categories: xx, xx, xx... . The key points are the summarization of the existing work. Do not show too much details. the details should be introduced in the related work Section. Then highlight the limitations and challenges, which should be consistent with our contributions}

%\subsubsection*{\textbf{Prior work}}
%Previous work often focused on only one aspect of intent discovery. For open intent discovery, Shi et al.\cite{shi2018auto} used an autoencoder to extract intent features and applies a hierarchical clustering approach to automatically label intents in unsupervised scenarios.  Shi et al.\cite{liu2021open} proposed an unsupervised clustering method that automatically extracts intent clusters from unlabelled data sets and uses dependency parsers to generate intent labels. Lin, Xu, and Zhang\cite{lin2020discovering}  proposed using pairwise similarity as a weakly supervised signal to discriminate intents when there is a limited amount of labeled data available. Zhang et al.\cite{zhang2021discovering} proposed a semi-supervised iterative clustering method that can effectively utilize a small amount of labeled data.  Shen et al.\cite{shen2021semi} proposed a semi-supervised framework using a combination of supervised contrast learning and unsupervised k-means clustering. These methods often adopt a pipeline approach where intent representation and clustering are treated as independent processes, and fail to capture the inherent connections between intent representation and clustering, leading to a misalignment between intent representations and clustering. Zhang et al.\cite{zhang2022new} uses a large amount of unlabeled data and externally labeled data for pre-training, which requires additional information and may cause an increase in computation cost.
 
Previous work only focused on only one aspect of intent discovery. For open intent discovery,  \cite{lin2020discovering}  proposed using pairwise similarity as a weakly supervised signal to discriminate intents when there is a limited amount of labeled data available. \cite{zhang2021discovering} proposed a semi-supervised iterative clustering method that can effectively utilize a small amount of labeled data.  \cite{shen2021semi} proposed a semi-supervised framework using a combination of supervised contrast learning and unsupervised k-means clustering. These methods often adopt a pipeline approach where intent representation and clustering are treated as independent processes, and fail to capture the inherent connections between intent representation and clustering, leading to a misalignment between intent representations and clustering.\cite{zhang2022new} uses a large amount of unlabeled data and externally labeled data for pre-training, which requires additional information and may cause an increase in computation cost.
For OOD intent discovery, previous works typically use a contrastive clustering\cite{li2021contrastive} framework. \cite{mou2022disentangled} proposed a multi-head contrast learning framework that maps sentence features to different feature spaces to disentangle knowledge. \cite{mou2022watch} proposed a unified K-nearest neighbor contrastive learning framework to alleviate the in-domain overfitting problem and mine true hard negative samples. 
They typically use a two-stage contrastive clustering approach, involving supervised pre-training and unsupervised clustering, and overlook the crucial supervised signals from IND samples in the clustering stage. 
%Moreover, they ignore the potential diversity of samples within the same class, leading to negative consequences on the quality of clustering results.
%\yx{give the full name of KCL and KCC}

%\subsubsection*{\textbf{Research problem and challenges}}
%Existing algorithms focus on analyzing explicit semantic information and performing classification tasks through semantic alignment, feature clustering, and contrastive clustering. However, further exploration of implicit information is necessary: (1) The existing methods face a bottleneck in simultaneously preserving the information of labeled data and adapting to unlabeled data. The main challenge is to strike a balance between relying heavily on prior knowledge and avoiding catastrophic forgetting, which can occur when labeled samples are disregarded during the training process. (2) In the process of intent discovery, a large amount of unlabeled data is often involved. Previously, the focus was solely on the semantic information of each unlabeled sample, while the potential connections between samples were overlooked.(3) The feature of cluster and the feature of instance are always extracted independently, despite the existence of a natural connection between them arising from their inclusion relationship.
\iffalse
While previous methods have achieved successful performance, several challenges in the field remain unexplored. 
One key challenge is to efficiently integrate labeled and unlabeled data for joint representation learning and clustering. 
%Some methods adopt a two-stage approach, segregating representation learning and clustering, introducing potential inefficiencies. Recently, there are approaches employing joint representation learning and clustering through contrastive clustering. However, they overlook the existing labeled data and only conduct clustering on unlabeled data. Furthermore, during contrastive learning, they usually rely on unsupervised contrastive samples which neglect potential positive or negative samples. 
Leveraging the labeled information is essential to facilitate the joint representation learning and clustering process. Considering that the number of labeled data is usually limited, it will bring the overfitting problem without careful design.  %Additionally, as model training progresses, it becomes imperative to effectively utilize confidently trained unlabeled data to identify potential contrastive samples during clustering.

Another critical challenge involves designing methods for efficient transfer learning between IND and OOD data.
%This aims to enhance the acquisition of new intent knowledge while preventing catastrophic forgetting of prior knowledge. 
Many existing methods train a classifier over prior knowledge and subsequently discard it, retaining only the feature extraction during the clustering stage with OOD samples. This necessitates the design of additional alignment strategies to maintain consistent cluster indices, potentially introducing noise if the alignment is suboptimal. 
%Thus there is an urgent need to develop proper methods that preserve prior knowledge while better adapting to new intent data, ensuring a seamless and effective transfer learning process.


Last but not least, previous works focus on either open intent discovery or OOD intent discovery.
%lacking a unified framework that can handle both tasks effectively. 
In real-world scenarios, task-based dialogue systems often face the situation for updates or migration. Open intent discovery is used to explore new intents for updates, while OOD intent discovery quickly clusters OOD intents for migration. Since we usually do not know the extent of change the system is facing, proposing a uniform intent discovery method that performs well in both scenarios is needed. 
\fi
%In pursuit of addressing these limitations, w
We propose a \textbf{P}seudo-\textbf{L}abel enhanced \textbf{P}rotypical \textbf{C}ontrastive \textbf{L}earning (PLPCL) model which is built upon contrastive clustering for joint representation learning and clustering. Our approach begins by pre-training the contrastive clustering model using labeled IND data. To effectively harness labeled information, we integrate IND samples with unlabeled data using a semi-supervised clustering strategy, employing distinct contrastive learning strategies for labeled and unlabeled data. To prevent overfitting and maximize the utilization of unlabeled data, we iteratively select reliable unlabeled samples with confident pseudo-labels. These reliable samples serve as potential positive/negative samples during contrastive learning, enhancing the overall contrastive clustering process.

To bridge the gap between IND and OOD data, we introduce a prototype learning strategy. It keeps prototype matrix by integrating instance and cluster features from both the IND and reliable unlabeled samples. 
%Specifically, each prototype is computed through the weighted merge of instances belonging to the specific prototype, continually updated throughout the learning process. 
%Notably, o
Our method seamlessly integrates contrastive clustering and prototypical learning, eliminating the need for an extra aligning module. This integration facilitates improved knowledge transfer from IND to OOD without discarding label information from IND samples. Furthermore, our framework is purposefully designed for uniform intent discovery, demonstrating effectiveness in both open-setting and OOD-setting scenarios. 



%In detail, we first use labeled data to pre-train the model. After that, different contrastive learning strategies are adopted for labeled and unlabeled data to extract clustering-friendly features and cluster prototypes are explicitly decoupled to increase inter-class distance. Contrastive learning and prototype learning are combined in this step, and the potential connection between clusters and instances is further mined. Moreover, our approach iteratively utilizes reliable pseudo-labels to expand the positive samples for clustering, while avoiding the introduction of intolerable noise. This step starts with confidence and goes beyond the inherent semantics of the text to explore its potential label information. Moreover, it is specifically designed for uniformed intent discovery, which can effectively adapt to both open-setting and OOD-setting.

%In summary, our proposed method strives to address the limitations of existing approaches, providing a robust and adaptable solution for joint representation learning and clustering. 
The contribution of our work is threefold:

\begin{itemize}
\item We introduce a novel method that leverages both labeled and unlabeled data through pseudo-label enhanced semi-supervised contrastive learning. This approach facilitates joint representation learning and clustering by effectively leveraging the whole data.
\item We propose a prototypical contrastive learning framework for uniformed intent discovery integrating prototypical learning and contrastive clustering utilizing labeled and unlabeled samples to bridge the gap between IND prior knowledge and OOD categories. 
\item We conduct extensive experiments on both OOD intent discovery and open intent discovery scenarios and the results demonstrate the effectiveness of our proposed method.
\end{itemize}

\iffalse
\begin{itemize}
\item Iteratively using reliable pseudo labels as positive samples in contrastive learning, effectively enhancing the supervisory signal.
\item Proposing contrastive learning of cluster prototypes to solve the isolation problem between instance-level and cluster-level contrastive heads.
\item Using a balanced combination of labeled and unlabeled data during the training stage helps prevent overconfidence and catastrophic forgetting.
\item Constructing a uniformed intent discovery model for both OOD intent discovery and open intent discovery.
\end{itemize}
\fi


